Penalized Parabolic Relaxation for Optimal Power Flow Problem

This paper is concerned with optimal power flow (OPF), which is the problem of optimizing the transmission of electricity in power systems. Our main contributions are as follows: (i) we propose a novel parabolic relaxation, which transforms non-convex OPF problems into convex quadratically-constrained quadratic programs (QCQPs) and can serve as an alternative to the common practice semidefinite programming (SDP) and second-order cone programming (SOCP) relaxations, (ii) we propose a penalization technique which is compatible with the SDP, SOCP, and parabolic relaxations and guarantees the recovery of feasible solutions for OPF, under certain assumptions. The proposed penalized convex relaxation can be used sequentially to find feasible and near-globally optimal solutions for challenging instances of OPF. Extensive numerical experiments on small and large-scale benchmark systems corroborate the efficacy of the proposed approach. By solving a few rounds of penalized convex relaxation, fully feasible solutions are obtained for benchmark test cases from [1]-[3] with as many as 13659 buses. In all cases, the solutions obtained are not more than 0.32% worse than the best-known solutions.

==> table_PARA.tex <==
\begin{table*}[!t]
\scriptsize
	\centering
	\caption{Parabolic results summary for IEEE, modified-IEEE  \cite{bukhsh2013local}, and European test cases.}
	\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Test Case} & \multicolumn{13}{c|}{Parabolic}\\
		\cline{2-14}
 		& $\mu$ & $\alpha$ & t(s) & $k_{f}$ & \%GFB & \%GFS & $k_{p}$ & \%GPB & \%GPS & $c_{f}$ & $c_{p}$ & $c_{g}$ & $lb$\\
		\hline
		\hline
        case6ww & 0.01 & 5 & -- & 2 & 0.01 & 0.01 & 3 & 0.00 & 0.00 & 3144.14 & 3143.98 & 3143.97 & 3143.97 \\ \hline
        case9 & 0.01 & 5 & -- & 1 & 0.24 & 0.24 & 9 & 0.00 & 0.00 & 5309.44 & 5296.77 & 5296.69 & 5296.69 \\ \hline
        case14 & 0.001 & 5 & -- & 1 & 9.60 & 9.60 & 38 & 0.01 & 0.01 & 8939.65 & 8082.61 & 8081.53 & 8081.53 \\ \hline
        case30 & 0.01 & 5 & -- & 2 & 2.02 & 2.02 & 29 & 0.02 & 0.02 & 588.76 & 577.00 & 576.89 & 576.89 \\  \hline
        case\_ieee30 & 0.001 & 5 & -- & 2 & 9.84 & 9.84 & 61 & 0.01 & 0.01 & 9877.99 & 8907.20 & 8906.14 & 8906.14 \\ \hline
        case39 & 0.01 & 10 & -- & 8 & 0.03 & 0.03 & 9 & 0.00 & 0.01 & 41875.98 & 41864.91 & 41864.18 & 41862.08 \\ \hline
        case57 & 0.01 & 10 & -- & 7 & 0.00 & 0.00 & 8 & 0.00 & 0.00 & 41739.41 & 41738.54 & 41737.79 & 41737.79 \\ \hline
        case118 & 0.001 & 5 & -- & 2 & 1.38 & 1.39 & 48 & 0.06 & 0.06 & 131477.75 & 129732.30 & 129660.69 & 129654.63 \\ \hline
        case300 & 0.001 & 10 & --- & 7 & 0.18 & 0.18 & 21 & 0.04 & 0.04 & 721016.22 & 719978.27 & 719725.08 & 719711.70 \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BUKHSH
        \hline
        case9mod & 0.0001 & 1 & -- & 9 & 0.48 & 11.27 & 22 & 0.00 & 10.84 & 3102.73 & 3087.91 & 3087.84 & 2753.04 \\ \hline
        case22loop & 0.01 & 1 & -- & 3 & 0.00 & 0.00 & 3 & 0.00 & 0.00 & 4538.92 & 4538.92 & 4538.80 & 4538.80 \\ \hline
        case30loop & 0.01 & 1 & -- & 1 & 0.04 & 0.04 & 12 & 0.01 & 0.01 & 2864.07 & 2863.38 & 2863.06 & 2863.06 \\ \hline
        case30loopmod & 0.01 & 1 & -- & 1 & 0.08 & 0.08 & 12 & 0.05 & 0.05 & 2864.07 & 2863.38 & 2861.88 & 2861.88 \\ \hline
        case39mod1 & 0.0001 & 5 & -- & 3 & 9.23 & 12.58 & 71 & 0.07 & 3.76 & 12359.36 & 11226.74 & 11219.00 & 10804.08 \\ \hline
        case39mod2 & 0.1 & 5 & -- & 3 & 0.07 & 0.22 & 9 & 0.03 & 0.18 & 942.41 & 942.04 & 941.74 & 940.34 \\ \hline
        case39mod3 & 0.01 & 5 & -- & 3 & 0.03 & 0.33 & 5 & 0.02 & 0.32 & 1890.56 & 1890.47 & 1890.05 & 1884.38 \\ \hline
        case39mod4 & 0.1 & 5 & -- & 5 & 1.31 & 1.32 & 25 & 0.01 & 0.02 & 564.53 & 557.20 & 557.14 & 557.08 \\ \hline
        case118mod & 0.001 & 5 & -- & 2 & 1.42 & 1.42 & 48 & 0.05 & 0.05 & 131494.32 & 129694.30 & 129625.03 & 129624.98 \\ \hline
        case300mod & 0.0001 & 5 & --- & 12 & 1.12 & 1.26 & 96 & 0.25 & 0.39 & 382834.75 & 379502.35 & 378541.74 & 378022.80 \\
 \hline
        case300mod1 & 0.001 & 5 & -- & 6 & -1.21 & 0.16 & 27 & -1.34 & 0.03 & 475397.79 & 474757.17 & 481126.61 & 474625.99 \\ \hline
		WB2 & 0.01 & 5 & -- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 877.78 & 877.78 & 877.78 & 877.78 \\
		\hline
		WB3 & 0.01 & 5 & -- & 2 & 0.04 & 0.04 & 10 & 0.01 & 0.01 & 417.44 & 417.29 & 417.25 & 417.25 \\
		\hline
		WB5 & 0.01 & 5 & -- & 21 & 0.00 & 0.00 & 21 & 0.00 & 0.00 & 946.58 & 946.58 & 946.58 & 946.54 \\
		\hline
		\textcolor{red}{WB5mod} & 0.01 & 5 & -- & 2 & 41.17 & 5.07 & 21 & 38.03 & 0.01 & 1561.43 & 1482.29 & 918.55 & 1482.22 \\
		\hline     
        \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% polish %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		case2383wp & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --  \\
		\hline
        case2736sp & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --  \\
		\hline
        case2737sop & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --  \\
		\hline
        case2746wop & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --   \\
		\hline
        case2746wp & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --  \\
		\hline
        case3012wp & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --   \\
		\hline
        case3120sp & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
		\hline
        case3375wp & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --  \\
		\hline
        \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% pegase %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		case89pegase & 0.01 & 10 & -- & 19 & 0.23 & 0.23 & 63 & 0.10 & 0.10 & 5833.19 & 5825.55 & 5819.81 & 5819.67 \\
		\hline
		case1354pegase & 0.001 & 5 & -- & 14 & -- & 0.34 & 14 & -- & 0.34 & 74311.50 & 74311.50 & -- & 74062.53 \\
		\hline
        case2869pegase & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --\\
		\hline
        case9241pegase & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
		\hline
        case13659pegase & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
		\hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% rte %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 		case1888rte & -- & -- & -- & -- & -- & -- & -- & --& -- & -- & -- & --  \\
% 		\hline
%         case1951rte & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% 		\hline
%         case2848rte & -- & -- & -- & -- & -- & -- & -- & --& -- & -- & -- & --  \\
% 		\hline
%         case2868rte & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% 		\hline
%         case6468rte & -- & -- & -- & -- & -- & -- & -- & --& -- & -- & -- & --  \\
% 		\hline
%         case6470rte & -- & -- & -- & -- & -- & -- & -- & --& -- & -- & -- & -- \\
% 		\hline
%         case6495rte & -- & -- & -- & -- & -- & -- & -- & --& -- & -- & -- & --  \\
% 		\hline
%         case6515rte & -- & -- & -- & -- & -- & -- & -- & --& -- & -- & -- & --  \\
%         \hline
%         \hline
	\end{tabular}
	\label{tab:PARA_tb_1}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t] 
\scriptsize
	\centering
	\caption{Parabolic results summary for NESTA test cases.}
	\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Test Case} & \multicolumn{13}{c|}{Parabolic}\\
		\cline{2-14}
 		& $\mu$ & $\alpha$ & t(s) & $k_{f}$ & \%GFB & \%GFS & $k_{p}$ & \%GPB & \%GPS & $c_{f}$ & $c_{p}$ & $c_{g}$ & $lb$\\

		\hline
		\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nesta %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs & 0.001 & 5 & --- & 1 & 47.38 & 47.38 & 10 & 0.00 & 0.00 & 297.28 & 156.43 & 156.43 & 156.43 \\ \hline
        nesta\_case5\_pjm & 0.0001 & 10 & --- & 1 & 2.47 & 7.56 & 45 & 0.07 & 5.28 & 17995.79 & 17563.32 & 17551.89 & 16635.78 \\ \hline
        nesta\_case6\_c & 0.1 & 1 & --- & 1 & 3.23 & 3.23 & 19 & -0.01 & -0.01 & 23.99 & 23.21 & 23.21 & 23.21 \\ \hline
        nesta\_case9\_wscc & 0.01 & 5 & --- & 1 & 0.24 & 0.24 & 9 & 0.00 & 0.00 & 5309.44 & 5296.77 & 5296.69 & 5296.69 \\ \hline
        nesta\_case14\_ieee & 0.01 & 5 & --- & 5 & 0.13 & 0.13 & 23 & 0.09 & 0.09 & 244.37 & 244.27 & 244.05 & 244.05 \\ \hline
        nesta\_case24\_ieee\_rts & 0.001 & 5 & --- & 4 & 0.03 & 0.03 & 7 & 0.00 & 0.00 & 63371.03 & 63352.72 & 63352.20 & 63352.20 \\ \hline
        nesta\_case29\_edin & 0.01 & 5 & --- & 4 & 0.36 & 0.36 & 36 & 0.01 & 0.01 & 30004.02 & 29898.72 & 29895.49 & 29895.49 \\ \hline
        nesta\_case30\_as & 0.01 & 5 & --- & 5 & 5.20 & 5.20 & 28 & 0.01 & 0.01 & 847.15 & 803.25 & 803.13 & 803.13 \\ \hline
        nesta\_case30\_fsr & 0.01 & 5 & --- & 2 & 2.03 & 2.03 & 30 & 0.02 & 0.02 & 587.67 & 575.88 & 575.77 & 575.77 \\ \hline
        nesta\_case30\_ieee & 0.01 & 5 & --- & 9 & 4.52 & 4.52 & 36 & 0.00 & 0.00 & 214.67 & 204.98 & 204.97 & 204.97 \\ \hline
        nesta\_case39\_epri & 0.001 & 5 & --- & 5 & 0.09 & 0.11 & 15 & 0.01 & 0.03 & 96593.28 & 96516.46 & 96505.52 & 96491.10 \\ \hline
        nesta\_case57\_ieee & 0.01 & 5 & --- & 3 & 4.03 & 4.03 & 35 & 0.02 & 0.02 & 1191.26 & 1143.45 & 1143.27 & 1143.27 \\ \hline
        nesta\_case73\_ieee\_rts & 0.001 & 5 & --- & 3 & 0.10 & 0.10 & 8 & 0.00 & 0.00 & 189953.82 & 189768.73 & 189764.08 & 189764.08 \\ \hline
        nesta\_case89\_pegase & 0.01 & 10 & --- & 19 & 0.23 & 0.23 & 63 & 0.10 & 0.10 & 5833.19 & 5825.55 & 5819.81 & 5819.67 \\ \hline
		\textcolor{orange}{nesta\_case118\_ieee} & 0.01 & 5 & --- & 2 & 14.21 & 14.26 & 80 & 0.33 & 0.39 & 4334.40 & 3730.87 & 3718.64 & 3716.25 \\
        \hline
        nesta\_case162\_ieee\_dtc & 0.001 & 5 & --- & 8 & 2.55 & 3.60 & 69 & 1.52 & 2.58 & 4340.82 & 4295.33 & 4230.23 & 4184.71 \\ \hline
        nesta\_case189\_edin & 0.01 & 1 & --- & 6 & 3.09 & 3.12 & 73 & 0.01 & 0.04 & 876.37 & 849.36 & 849.29 & 849.02 \\\hline
		\textcolor{orange}{nesta\_case300\_ieee}& 0.01 & 10 & --- & 75 & 1.20 & 1.27 & 80 & 1.16 & 1.24 & 17095.69 & 17089.87 & 16891.28 & 16878.14 \\ \hline
		\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nesta_api %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs\_\_api & 0.01 & 5 & --- & 5 & -0.02 & 0.06 & 7 & -0.08 & 0.00 & 767.13 & 766.68 & 767.27 & 766.67 \\ \hline
        nesta\_case5\_pjm\_\_api & 0.01 & 5 & --- & 4 & -0.03 & 0.05 & 8 & -0.07 & 0.00 & 2997.72 & 2996.32 & 2998.54 & 2996.32 \\ \hline
        nesta\_case6\_c\_\_api & 0.01 & 5 & --- & 3 & 0.29 & 0.35 & 13 & -0.07 & -0.00 & 816.76 & 813.87 & 814.40 & 813.87  \\ \hline
        nesta\_case9\_wscc\_\_api & 0.01 & 5 & --- & 2 & -0.01 & 0.05 & 4 & -0.06 & 0.00 & 656.55 & 656.23 & 656.60 & 656.23\\ \hline
        nesta\_case14\_ieee\_\_api & 0.01 & 5 & --- & 18 & -0.04 & 0.09 & 31 & -0.12 & 0.01 & 325.43 & 325.16 & 325.56 & 325.13 \\ \hline
        \textcolor{orange}{nesta\_case24\_ieee\_rts\_\_api} & 0.001 & 5 & --- & 6 & 3.66 & 4.98 & 80 & 0.23 & 1.60 & 6665.18 & 6435.89 & 6421.37 & 6333.07  \\\hline
        nesta\_case29\_edin\_\_api & 0.001 & 5 & --- & 35 & -0.15 & 0.02 & 35 & -0.15 & 0.02 & 295339.73 & 295339.73 & 295782.68 & 295291.22\\\hline
        nesta\_case30\_as\_\_api & 0.01 & 10 & --- & 17 & 0.17 & 0.35 & 35 & -0.18 & 0.00 & 572.08 & 570.10 & 571.13 & 570.08  \\ \hline
        \textcolor{orange}{nesta\_case30\_fsr\_\_api} & 0.0001 & 5 & --- & 9 & 3.05 & 14.56 & 80 & -1.00 & 11.00 & 383.83 & 368.47 & 372.14 & 327.95 \\ \hline
        nesta\_case30\_ieee\_\_api & 0.01 & 5 & --- & 45 & -0.13 & 0.00 & 45 & -0.13 & 0.00 & 414.99 & 414.99 & 415.53 & 414.99 \\ \hline
        nesta\_case39\_epri\_\_api & 0.01 & 10 & --- & 27 & -0.06 & 0.02 & 28 & -0.08 & -0.00 & 7462.11 & 7460.37 & 7466.25 & 7460.37  \\ \hline
        nesta\_case57\_ieee\_\_api& 0.01 & 5 & --- & 2 & 2.76 & 2.84 & 44 & 0.01 & 0.09 & 1471.30 & 1430.83 & 1430.65 & 1429.51 \\ \hline
        \textcolor{orange}{nesta\_case73\_ieee\_rts\_\_api}& 0.0001 & 5 & --- & 7 & 4.90 & 9.57 & 80 & 1.25 & 6.10 & 21161.15 & 20379.49 & 20123.98 & 19135.79 \\\hline
        nesta\_case89\_pegase\_\_api& -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \hline
        \textcolor{orange}{nesta\_case162\_ieee\_dtc\_\_api} & 0.001 & 5 & --- & 61 & 0.17 & 1.10 & 80 & 0.03 & 0.95 & 6122.32 & 6113.44 & 6111.68 & 6055.28 \\\hline
        \textcolor{orange}{nesta\_case300\_ieee\_\_api}&  0.01 & 5 & --- & 9 & -11.94 & 2.74 & 80 & -14.73 & 0.32 & 20426.33 & 19930.15 & 22866.01 & 19866.78  \\ \hline
        \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nesta_sad %%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs\_\_sad & 0.01 & 10 & --- & 1 & 0.59 & 3.15 & 2 & -2.59 & 0.05 & 325.94 & 315.84 & 324.02 & 315.69 \\ \hline
        nesta\_case5\_pjm\_\_api& 0.0001 & 5 & --- & 3 & -0.79 & 0.39 & 5 & -1.17 & 0.01 & 26216.91 & 26117.59 & 26423.32 & 26115.20 \\\hline
        nesta\_case6\_c\_\_sad& 0.001 & 5 & --- & 2 & 0.10 & 0.30 & 2 & 0.10 & 0.30 & 24.45 & 24.45 & 24.43 & 24.38 \\\hline
        nesta\_case6\_ww\_\_sad & 0.001 & 5 & --- & 1 & 0.04 & 0.14 & 3 & -0.10 & 0.00 & 3150.82 & 3146.27 & 3149.51 & 3146.27 \\\hline
        nesta\_case9\_wscc\_\_sad & 0.001 & 5 & --- & 2 & -0.78 & 0.34 & 4 & -1.12 & 0.00 & 5547.02 & 5528.28 & 5590.09 & 5528.26\\\hline
        nesta\_case14\_ieee\_\_sad& 0.01 & 5 & --- & 5 & 0.09 & 0.13 & 23 & 0.05 & 0.09 & 244.37 & 244.27 & 244.15 & 244.05 \\\hline
        nesta\_case24\_ieee\_rts\_\_sad & 0.0001 & 5 & --- & 2 & -0.48 & 7.34 & 5 & -3.71 & 4.36 & 79421.48 & 76948.50 & 79804.96 & 73591.73 \\\hline
        nesta\_case29\_edin\_\_sad & 0.0001 & 10 & --- & 36 & -10.93 & 22.43 & 92 & -13.29 & 20.77 & 42310.39 & 41426.40 & 46933.26 & 32821.76 \\\hline
        nesta\_case30\_as\_\_sad& 0.01 & 10 & --- & 4 & 0.81 & 2.88 & 15 & -1.89 & 0.24 & 921.90 & 897.50 & 914.44 & 895.34 \\\hline
        nesta\_case30\_fsr\_\_sad& 0.01 & 5 & --- & 7 & 0.04 & 0.23 & 16 & -0.16 & 0.02 & 577.99 & 576.80 & 577.73 & 576.68\\\hline
        nesta\_case30\_ieee\_\_sad& 0.01 & 5 & --- & 9 & 4.45 & 4.52 & 36 & -0.07 & 0.00 & 214.67 & 204.98 & 205.11 & 204.97 \\\hline
        nesta\_case39\_epri\_\_sad& 0.001 & 5 & --- & 5 & -0.44 & 0.10 & 6 & -0.49 & 0.06 & 96789.96 & 96749.58 & 97219.04 & 96692.45 \\\hline
        nesta\_case57\_ieee\_\_sad & 0.01 & 5 & --- & 6 & 2.43 & 2.48 & 30 & -0.04 & 0.02 & 1172.32 & 1143.46 & 1143.88 & 1143.27  \\\hline
        nesta\_case73\_ieee\_rts\_\_sad& 0.0001 & 5 & --- & 2 & 1.65 & 7.40 & 6 & -3.27 & 2.77 & 239181.30 & 227787.62 & 235241.70 & 221480.59 \\\hline
		nesta\_case89\_pegase\_\_sad& 0.01 & 10 & --- & 76 & -0.05 & 0.08 & 76 & -0.05 & 0.08 & 5824.29 & 5824.29 & 5827.01 & 5819.67 \\\hline
        nesta\_case118\_ieee\_\_sad& 0.01 & 5 & --- & 24 & -4.83 & 3.89 & 68 & -5.23 & 3.53 & 4124.80 & 4109.37 & 4324.17 & 3964.14 \\\hline
        \textcolor{orange}{nesta\_case162\_ieee\_dtc\_\_sad}& 0.001 & 5 & --- & 11 & -0.47 & 3.41 & 100 & -1.16 & 2.75 & 4348.59 & 4319.21 & 4369.19 & 4200.52 \\\hline
        \textcolor{orange}{nesta\_case189\_edin\_\_sad}& 0.01 & 5 & --- & 12 & -2.84 & 3.53 & 100 & -5.13 & 1.38 & 889.37 & 869.98 & 914.61 & 858.01 \\\hline
        \textcolor{orange}{nesta\_case300\_ieee\_\_sad} & 0.01 & 10 & --- & 30 & 1.47 & 1.64 & 100 & 0.96 & 1.13 & 17162.76 & 17074.41 & 16910.23 & 16880.74 \\\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\end{tabular}
	\label{tab:PARA_tb_2}
\end{table*}

==> table_SDP.tex <==
\begin{table*}[!t]
\scriptsize
	\centering
	\caption{SDP results summary for IEEE, modified-IEEE  \cite{bukhsh2013local}, and European test cases.}
	\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Test Case} & \multicolumn{13}{c|}{SDP}\\
		\cline{2-14}
 		& $\mu$ & $\alpha$ & t(s) & $k_{f}$ & \%GFB & \%GFS & $k_{p}$ & \%GPB & \%GPS & $c_{f}$ & $c_{p}$ & $c_{g}$ & $lb$\\
		\hline
		\hline
        case6ww & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 3143.98 & 3143.98 & 3143.97 & 3143.97 \\ \hline
        case9 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 5296.69 & 5296.69 & 5296.69 & 5296.69 \\ \hline
        case14 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 2 & 0.00 & 0.00 & 8081.74 & 8081.53 & 8081.53 & 8081.53 \\ \hline
        case30 & 0.1 & 1 & --- & 1 & 0.10 & 0.10 & 3 & 0.00 & 0.00 & 577.45 & 576.90 & 576.89 & 576.89 \\ \hline
        case\_ieee30 & 0.1 & 1 & --- & 1 & 0.01 & 0.01 & 2 & 0.00 & 0.00 & 8907.03 & 8906.14 & 8906.14 & 8906.14 \\ \hline
        case39 & 0.1 & 1 & --- & 1 & 0.00 & 0.01 & 1 & 0.00 & 0.01 & 41864.28 & 41864.28 & 41864.18 & 41862.08 \\ \hline
        case57 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 41737.93 & 41737.93 & 41737.79 & 41737.79 \\ \hline
        case118 & 0.1 & 1 & --- & 1 & 0.00 & 0.01 & 2 & 0.00 & 0.00 & 129665.94 & 129660.75 & 129660.69 & 129654.63 \\ \hline
		case300 & 0.001 & 1 & --- & 1 & 0.60 & 0.60 & 7 & 0.02 & 0.02 & 724036.60 & 719848.70 & 719725.08 & 719711.70 \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BUKHSH
\hline
		case9mod & 0.0001 & 1 & --- & 5 & 0.89 & 11.63 & 19 & 0.00 & 10.85 & 3115.43 & 3087.97 & 3087.84 & 2753.04 \\ \hline
        case22loop & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 4538.84 & 4538.84 & 4538.80 & 4538.80 \\ \hline
        case30loop & 0.1 & 1 & --- & 1 & 0.02 & 0.02 & 2 & 0.00 & 0.00 & 2863.52 & 2863.07 & 2863.06 & 2863.06 \\ \hline
        case30loopmod & 0.1 & 1 & --- & 1 & 0.06 & 0.06 & 5 & 0.00 & 0.00 & 2863.52 & 2861.88 & 2861.88 & 2861.88 \\ \hline
        case39mod1 & 0.0001 & 1 & --- & 3 & 9.54 & 12.88 & 66 & 0.08 & 3.77 & 12401.57 & 11227.65 & 11219 & 10804.08 \\ \hline
        case39mod2 & 0.1 & 1 & --- & 3 & 0.04 & 0.19 & 5 & 0.03 & 0.18 & 942.11 & 942.06 & 941.74 & 940.34 \\ \hline
        case39mod3 & 0.1 & 1 & --- & 2 & -0.01 & 0.29 & 8 & -0.03 & 0.27 & 1889.93 & 1889.48 & 1890.05 & 1884.38 \\ \hline
        case39mod4 & 0.1 & 1 & --- & 1 & 2.15 & 2.16 & 7 & 0.01 & 0.02 & 569.36 & 557.19 & 557.14 & 557.08 \\ \hline
        case118mod & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 2 & 0.00 & 0.00 & 129630.05 & 129625.08 & 129625.03 & 129624.98 \\ \hline
		case300mod & 0.0001 & 1 & --- & 6 & 0.89 & 1.03 & 63 & 0.12 & 0.25 & 381943.07 & 378985.01 & 378541.74 & 378022.80 \\ \hline
        case300mod1 & 0.1 & 1 & --- & 1 & -1.37 & 0.00 & 2 & -1.37 & 0.00 & 474640.83 & 474629.02 & 481126.61 & 474625.99 \\ \hline 
% 		WB2& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & 877.78 & 877.78 \\
% 		\hline
        WB3 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 417.25 & 417.25 & 417.25 & 417.25 \\
		\hline
		WB5 & 0.1 & 5 & --- & 7 & 0.00 & 0.00 & 7 & 0.00 & 0.00 & 946.58 & 946.58 & 946.58 & 946.54 \\
		\hline
		\textcolor{red}{WB5mod} & 0.1 & 1 & --- & 1 & 38.10 & 0.11 & 2 & 38.03 & 0.00 & 1483.85 & 1482.24 & 918.55 & 1482.22 \\ \hline     
        \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% pegase %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		case89pegase & 0.01 & 1 & --- & 1 & 0.11 & 0.11 & 18 & 0.03 & 0.03 & 5826.37 & 5821.65 & 5819.81 & 5819.67 \\ \hline
	case1354pegase & 0.01 & 1 & --- & 1 & --- & 0.16 & 17 & --- & 0.08 & 74180.05 & 74121.52 & --- & 74062.53 \\  \hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% rte %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 		case1888rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case1951rte & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
%         case2848rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case2868rte & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
%         case6468rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case6470rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & --- \\
% 		\hline
%         case6495rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case6515rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
%         \hline
%         \hline
	\end{tabular}
	\label{tab:SDP_tb_1}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t] 
\scriptsize
	\centering
	\caption{SDP results summary for NESTA test cases.}
	\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Test Case} & \multicolumn{13}{c|}{SDP}\\
		\cline{2-14}
 		& $\mu$ & $\alpha$ & t(s) & $k_{f}$ & \%GFB & \%GFS & $k_{p}$ & \%GPB & \%GPS & $c_{f}$ & $c_{p}$ & $c_{g}$ & $lb$\\
		\hline
		\hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 156.43 & 156.43 & 156.43 & 156.43 \\
		\hline
		nesta\_case5\_pjm & 0.001 & 1 & --- & 1 & 0.21 & 5.42 & 5 & 0.00 & 5.22 & 17588.34 & 17551.89 & 17551.89 & 16635.78 \\
		\hline
        nesta\_case6\_c & 0.1 & 1 & --- & 1 & 3.25 & 3.25 & 3 & 0.17 & 0.17 & 23.99 & 23.25 & 23.21 & 23.21 \\
		\hline
        nesta\_case9\_wscc & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 5296.69 & 5296.69 & 5296.69 & 5296.69  \\
		\hline
        nesta\_case14\_ieee  & 0.1 & 1 & --- & 1 & 0.11 & 0.11 & 5 & 0.00 & 0.00 & 244.31 & 244.05 & 244.05 & 244.05\\
		\hline
        nesta\_case24\_ieee\_rts & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 63352.23 & 63352.23 & 63352.20 & 63352.20 \\
		\hline
		nesta\_case29\_edin & 0.1 & 1 & --- & 1 & 0.12 & 0.12 & 4 & 0.00 & 0.00 & 29929.97 & 29895.92 & 29895.49 & 29895.49 \\
		\hline
		nesta\_case30\_as & 0.1 & 1 & --- & 1 & 0.39 & 0.39 & 3 & 0.00 & 0.00 & 806.30 & 803.14 & 803.13 & 803.13 \\
		\hline
		nesta\_case30\_fsr & 0.1 & 1 & --- & 1 & 0.08 & 0.08 & 3 & 0.00 & 0.00 & 576.24 & 575.77 & 575.77 & 575.77\\
		\hline
		nesta\_case30\_ieee & 0.1 & 1 & --- & 1 & 0.27 & 0.27 & 3 & 0.00 & 0.00 & 205.53 & 204.97 & 204.97 & 204.97 \\
		\hline
		nesta\_case39\_epri & 0.01 & 1 & --- & 1 & 0.01 & 0.02 & 2 & 0.00 & 0.02 & 96514.04 & 96505.78 & 96505.52 & 96491.10  \\
		\hline
		nesta\_case57\_ieee & 0.1 & 1 & --- & 1 & 0.10 & 0.10 & 3 & 0.00 & 0.00 & 1144.41 & 1143.29 & 1143.27 & 1143.27 \\
		\hline
		nesta\_case73\_ieee\_rts & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 189764.20 & 189764.20 & 189764.08 & 189764.08  \\
		\hline
		nesta\_case89\_pegase & 0.1 & 5 & --- & 30 & 0.00 & 0.01 & 31 & 0.00 & 0.00 & 5820.05 & 5819.89 & 5819.81 & 5819.67  \\
		\hline
		nesta\_case118\_ieee & 0.1 & 1 & --- & 1 & 2.34 & 2.40 & 8 & 0.00 & 0.07 & 3807.56 & 3718.74 & 3718.64 & 3716.25 \\
		\hline
		\textcolor{orange}{nesta\_case162\_ieee\_dtc}& 0.01 & 5 & --- & 9 & 1.47 & 2.53 & 50 & 0.89 & 1.96 & 4293.40 & 4268.35 & 4230.23 & 4184.71  \\
		\hline
		\textcolor{orange}{nesta\_case300\_ieee} & 0.01 & 1 & --- & 1 & 3.91 & 3.98 & 50 & 0.02 & 0.09 & 17578.10 & 16893.91 & 16891.28 & 16878.14  \\
		\hline
% 		nesta\_case1354\_pegase& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case1460wp\_eir & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2224\_edin  & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2383wp\_mp & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2736sp\_mp & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2737sop\_mp & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\ \hline
        \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nesta %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs\_\_api & 0.1 & 1 & --- & 1 & -0.08 & 0.00 & 1 & -0.08 & 0.00 & 766.67 & 766.67 & 767.27 & 766.67\\
		\hline
		nesta\_case5\_pjm\_\_api & 0.1 & 1 & --- & 1 & -0.07 & 0.00 & 1 & -0.07 & 0.00 & 2996.38 & 2996.38 & 2998.54 & 2996.32  \\
		\hline
        nesta\_case6\_c\_\_api & 0.1 & 1 & --- & 1 & -0.03 & 0.04 & 2 & -0.07 & 0.00 & 814.18 & 813.87 & 814.40 & 813.87  \\
		\hline
        nesta\_case9\_wscc\_\_api & 0.1 & 1 & --- & 1 & -0.05 & 0.00 & 1 & -0.05 & 0.00 & 656.24 & 656.24 & 656.60 & 656.23\\
		\hline
        nesta\_case14\_ieee\_\_api  & 0.1 & 1 & --- & 1 & -0.10 & 0.04 & 3 & -0.13 & 0.00 & 325.25 & 325.13 & 325.56 & 325.13\\
		\hline
        nesta\_case24\_ieee\_rts\_\_api & 0.01 & 1 & --- & 16 & 0.08 & 1.46 & 16 & 0.08 & 1.46 & 6426.72 & 6426.72 & 6421.37 & 6333.07  \\
		\hline
		nesta\_case29\_edin\_\_api & 0.1 & 1 & --- & 1 & -0.16 & 0.01 & 2 & -0.17 & 0.00 & 295309.44 & 295295.18 & 295782.68 & 295291.22 \\
		\hline
		nesta\_case30\_as\_\_api & 0.1 & 1 & --- & 1 & 0.20 & 0.38 & 2 & -0.18 & 0.00 & 572.26 & 570.09 & 571.13 & 570.08\\
		\hline
		nesta\_case30\_fsr\_\_api & 0.01 & 5 & --- & 1 & -0.49 & 11.45 & 12 & -1.52 & 10.54 & 370.34 & 366.58 & 372.14 & 327.95 \\
		\hline
		nesta\_case30\_ieee\_\_api & 0.1 & 1 & --- & 1 & -0.13 & 0.00 & 2 & -0.13 & 0.00 & 415.00 & 414.99 & 415.53 & 414.99 \\
		\hline
		nesta\_case39\_epri\_\_api & 0.1 & 1 & --- & 1 & -0.07 & 0.01 & 2 & -0.08 & 0.00 & 7461.08 & 7460.37 & 7466.25 & 7460.37  \\
		\hline
		nesta\_case57\_ieee\_\_api & 0.1 & 1 & --- & 1 & 0.36 & 0.44 & 3 & 0.00 & 0.08 & 1435.82 & 1430.67 & 1430.65 & 1429.51  \\
		\hline
		\textcolor{orange}{nesta\_case73\_ieee\_rts\_\_api} & 0.001 & 1 & --- & 3 & 1.33 & 6.18 & 50 & -0.55 & 4.39 & 20395.36 & 20014.18 & 20123.98 & 19135.79 \\
		\hline
		nesta\_case89\_pegase\_\_api & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
		\hline
		nesta\_case118\_ieee\_\_api & 0.001 & 1 & --- & 3 & 0.69 & 32.30 & 38 & -0.50 & 31.48 & 10397.19 & 10273.55 & 10325.27 & 7039.38\\
		\hline
		nesta\_case162\_ieee\_dtc\_\_api& 0.001 & 1 & --- & 8 & 0.17 & 1.09 & 30 & -0.05 & 0.87 & 6122.08 & 6108.73 & 6111.68 & 6055.28 \\
		\hline
		nesta\_case189\_edin\_\_api& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
		\hline
		nesta\_case300\_ieee\_\_api & 0.01 & 1 & --- & 1 & -8.45 & 5.77 & 50 & -15.02 & 0.06 & 21083.92 & 19879.19 & 22866.01 & 19866.78 \\
		\hline
% 		nesta\_case1354\_pegase\_\_api& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case1460wp\_eir\_\_api & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2224\_edin\_\_api  & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2383wp\_mp\_\_api & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2736sp\_mp\_\_api & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2737sop\_mp\_\_api & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\	\hline
        \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
        nesta\_case4\_gs\_\_sad & 0.1 & 1 & --- & 1 & -2.59 & 0.05 & 1 & -2.59 & 0.05 & 315.84 & 315.84 & 324.02 & 315.69\\
		\hline
		nesta\_case5\_pjm\_\_sad & 0.1 & 1 & --- & 1 & -1.18 & 0.00 & 1 & -1.18 & 0.00 & 26115.22 & 26115.22 & 26423.32 & 26115.20  \\
		\hline
        nesta\_case6\_c\_\_sad  & 0.1 & 1 & --- & 1 & 0.08 & 0.29 & 5 & -0.21 & 0.00 & 24.45 & 24.38 & 24.43 & 24.38 \\
		\hline
        nesta\_case6\_ww\_\_sad & 0.1 & 1 & --- & 1 & -0.10 & 0.00 & 1 & -0.10 & 0.00 & 3146.27 & 3146.27 & 3149.51 & 3146.27 \\
		\hline
        nesta\_case9\_wscc\_\_sad & 0.1 & 1 & --- & 1 & -1.12 & 0.00 & 1 & -1.12 & 0.00 & 5528.26 & 5528.26 & 5590.09 & 5528.26  \\
		\hline
        nesta\_case14\_ieee\_\_sad & 0.1 & 1 & --- & 1 & 0.07 & 0.11 & 5 & -0.04 & 0.00 & 244.31 & 244.05 & 244.15 & 244.05 \\
		\hline
        nesta\_case24\_ieee\_rts\_\_sad & 0.001 & 1 & --- & 1 & -3.72 & 4.36 & 2 & -3.72 & 4.36 & 76945.09 & 76943.35 & 79804.96 & 73591.73 \\
		\hline
		nesta\_case29\_edin\_\_sad & 0.001 & 1 & --- & 1 & -8.11 & 24.39 & 23 & -13.73 & 20.46 & 43411.86 & 41266.93 & 46933.26 & 32821.76 \\
		\hline
		nesta\_case30\_as\_\_sad  & 0.1 & 5 & --- & 3 & -1.89 & 0.24 & 3 & -1.89 & 0.24 & 897.49 & 897.49 & 914.44 & 895.34\\
		\hline
		nesta\_case30\_fsr\_\_sad & 0.1 & 1 & --- & 1 & -0.14 & 0.04 & 2 & -0.16 & 0.02 & 576.90 & 576.79 & 577.73 & 576.68 \\
		\hline
		nesta\_case30\_ieee\_\_sad  & 0.1 & 1 & --- & 1 & 0.20 & 0.27 & 3 & -0.07 & 0.00 & 205.53 & 204.97 & 205.11 & 204.97 \\
		\hline
		nesta\_case39\_epri\_\_sad & 0.01 & 1 & --- & 1 & -0.49 & 0.06 & 2 & -0.49 & 0.05 & 96749.21 & 96745.01 & 97219.04 & 96692.45\\
		\hline
		nesta\_case57\_ieee\_\_sad & 0.1 & 1 & --- & 1 & 0.05 & 0.10 & 3 & -0.05 & 0.00 & 1144.41 & 1143.29 & 1143.88 & 1143.27 \\
		\hline
		nesta\_case73\_ieee\_rts\_\_sad & 0.001 & 1 & --- & 1 & -3.28 & 2.76 & 2 & -3.29 & 2.75 & 227766.33 & 227752.06 & 235241.70 & 221480.59 \\
		\hline
		nesta\_case89\_pegase\_\_sad & 0.1 & 5 & --- & 1 & 0.06 & 0.18 & 14 & -0.11 & 0.01 & 5830.36 & 5820.46 & 5827.01 & 5819.67 \\
		\hline
		nesta\_case118\_ieee\_\_sad & 0.1 & 5 & --- & 2 & -4.38 & 4.31 & 15 & -5.29 & 3.48 & 4142.82 & 4107.05 & 4324.17 & 3964.14 \\
		\hline
		\textcolor{orange}{nesta\_case162\_ieee\_dtc\_\_sad} & 0.001 & 1 & --- & 43 & -1.46 & 2.46 & 50 & -1.78 & 2.15 & 4306.36 & 4292.71 & 4369.19 & 4200.52 \\
		\hline
		nesta\_case189\_edin\_\_sad & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
		\hline
		nesta\_case300\_ieee\_\_sad & 0.01 & 1 & --- & 1 & 3.76 & 3.93 & 49 & -0.08 & 0.09 & 17570.81 & 16896.67 & 16910.23 & 16880.74 \\
		\hline
% 		nesta\_case1354\_pegase\_\_sad & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case1460wp\_eir\_\_sad & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2224\_edin\_\_sad  & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2383wp\_mp\_\_sad & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2736sp\_mp\_\_sad & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
% 		nesta\_case2737sop\_mp\_\_sad & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\ \hline
	\end{tabular}
	\label{tab:NESTA_testcases}
\end{table*}

==> table_SOCP.tex <==
\begin{table*}[!t]
\scriptsize
	\centering
	\caption{SOCP results summary for IEEE, modified-IEEE  \cite{bukhsh2013local}, \matpower, and PEGASE test cases.}
	\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Test Case} & \multicolumn{13}{c|}{SOCP}\\
		\cline{2-14}
 		& $\mu$ & $\alpha$ & t(s) & $k_{f}$ & \%GFB & \%GFS & $k_{p}$ & \%GPB & \%GPS & $c_{f}$ & $c_{p}$ & $c_{g}$ & $lb$\\
		\hline
		\hline
		case6ww & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 3143.98 & 3143.98 & 3143.97 & 3143.97 \\ \hline
		case9 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 5296.69 & 5296.69 & 5296.69 & 5296.69 \\ \hline
		case14 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 2 & 0.00 & 0.00 & 8081.74 & 8081.53 & 8081.53 & 8081.53 \\ \hline
		case30 & 0.1 & 1 & --- & 1 & 0.10 & 0.10 & 3 & 0.00 & 0.00 & 577.45 & 576.90 & 576.89 & 576.89 \\ \hline
		case\_ieee30 & 0.1 & 1 & --- & 1 & 0.01 & 0.01 & 2 & 0.00 & 0.00 & 8907.03 & 8906.14 & 8906.14 & 8906.14 \\ \hline
		case39 & 0.1 & 1 & --- & 1 & 0.00 & 0.01 & 1 & 0.00 & 0.01 & 41864.28 & 41864.28 & 41864.18 & 41862.08 \\ \hline
		case57 & 0.1 & 1 & --- & 2 & 0.00 & 0.00 & 2 & 0.00 & 0.00 & 41737.79 & 41737.79 & 41737.79 & 41737.79 \\ \hline
		case118 & 0.1 & 5 & --- & 1 & 0.05 & 0.06 & 3 & 0.00 & 0.01 & 129728.36 & 129661.77 & 129660.69 & 129654.63 \\ \hline
		case300 & 0.01 & 1 & --- & 1 & 0.03 & 0.03 & 3 & 0.00 & 0.01 & 719956.63 & 719753.51 & 719725.08 & 719711.70 \\ 
    	\hline
        \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BUKHSH %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        case9mod & 0.0001 & 1 & --- & 5 & 0.89 & 11.63 & 19 & 0.00 & 10.85 & 3115.43 & 3087.97 & 3087.84 & 2753.04 \\ \hline
        case22loop & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 4538.84 & 4538.84 & 4538.80 & 4538.80 \\ \hline
        case30loop & 0.1 & 1 & --- & 1 & 0.02 & 0.02 & 2 & 0.00 & 0.00 & 2863.52 & 2863.07 & 2863.06 & 2863.06 \\ \hline
        case30loopmod & 0.1 & 1 & --- & 1 & 0.06 & 0.06 & 5 & 0.00 & 0.00 & 2863.52 & 2861.88 & 2861.88 & 2861.88 \\ \hline
        case39mod1 & 0.0001 & 1 & --- & 2 & 6.32 & 9.78 & 47 & 0.04 & 3.74 & 11975.72 & 11223.42 & 11219.00 & 10804.08 \\ \hline
        case39mod2 & 0.1 & 1 & --- & 3 & 0.04 & 0.19 & 5 & 0.03 & 0.18 & 942.11 & 942.06 & 941.74 & 940.34 \\ \hline
        case39mod3 & 0.1 & 1 & --- & 2 & -0.01 & 0.29 & 8 & -0.03 & 0.27 & 1889.93 & 1889.48 & 1890.05 & 1884.38 \\ \hline
        case39mod4 & 0.1 & 1 & --- & 1 & 2.15 & 2.16 & 7 & 0.01 & 0.02 & 569.36 & 557.19 & 557.14 & 557.08 \\ \hline
        case118mod & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 2 & 0.00 & 0.00 & 129630.05 & 129625.08 & 129625.03 & 129624.98 \\ \hline
        case118mod1 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 2 & 0.00 & 0.00 & 85990.38 & 85987.86 & 85987.59 & 85987.27 \\
		\hline
        case300mod & 0.0001 & 1 & --- & 6 & 0.89 & 1.03 & 63 & 0.12 & 0.25 & 381943.15 & 378985.01 & 378541.74 & 378022.80 \\
\hline
        case300mod1 & 0.01 & 1 & --- & 2 & -1.35 & 0.02 & 4 & -1.37 & 0.00 & 474714.17 & 474646.50 & 481126.61 & 474625.99 \\ \hline
        WB2 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 877.78 & 877.78 & 877.78 & 877.78\\ \hline % baghiye parametra kollan fail mikone! 
        WB3 & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 417.25 & 417.25 & 417.25 & 417.25 \\ \hline
        WB5 & 0.01 & 1 & --- & 7 & 0.00 & 0.00 & 7 & 0.00 & 0.00 & 946.58 & 946.58 & 946.58 & 946.54 \\ \hline
        \textcolor{red}{WB5mod} & 0.1 & 1 & --- & 1 & 38.10 & 0.11 & 2 & 38.03 & 0.00 & 1483.85 & 1482.24 & 918.55 & 1482.22 \\ \hline  %lower bound chera!! bukhsh chera!!
        \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% polish %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\textcolor{orange}{case2383wp} & 0.001 & 5 & --- & 6 & 2.82 & 3.20 & 50 & 0.24 & 0.62 & 1922755.35 & 1872990.66 & 1868511.78 & 1861288.58\\
		\hline
        case2736sp & 0.01 & 5 & --- & 3 & 0.52 & 0.55 & 10 & 0.00 & 0.03 & 1314736.56 & 1307931.17 & 1307883.11 & 1307497.42 \\%300iter
		\hline
        case2737sop & 0.01 & 5 & --- & 4 & 0.18 & 0.28 & 18 & 0.01 & 0.10 & 779051.24 & 777689.24 & 777629.29 & 776887.84 \\%300iter
		\hline
        case2746wop & 0.01 & 5 & --- & 4 & 0.61 & 0.62 & 12 & 0.00 & 0.01 & 1215725.81 & 1208335.47 & 1208279.78 & 1208160.28 \\%300iter
		\hline
        \textcolor{orange}{case2746wp} & 0.001 & 5 & --- & 6 & 2.54 & 2.59 & 48 & 0.15 & 0.20 & 1674260.81 & 1634276.04 & 1631775.07 & 1630942.52 \\ %50 iteration
		\hline
		\textcolor{orange}{case3012wp} & 0.0001 & 1 & --- & 5 & 3.07 & 3.25 & 50 & 0.16 & 0.34 & 2673770.64 & 2595747.40 & 2591706.52 & 2586830.93\\
\hline
		case3120sp & 0.001 & 1 & --- & 2 & 2.37 & 2.47 & 15 & 0.00 & 0.10 & 2194754.80 & 2142759.85 & 2142703.73 & 2140555.87 \\
\hline
		\textcolor{orange}{case3375wp} & 0.0001 & 1 & --- & 5 & 1.59 & 1.66 & 50 & 0.10 & 0.16 & 7532103.17 & 7419319.65 & 7412030.61 & 7407349.49 \\ \hline
        \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RTE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        case1888rte & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  \\ \hline
        case1951rte & 0.01 & 1 & --- & 2 & --- & 0.11 & 13 & --- & 0.07 & 81818.97 & 81791.11 & --- & 81731.94 \\ \hline
        case2848rte & 0.01 & 5 & --- & 2 & --- & 0.17 & 11 & --- & 0.15 & 53096.62 & 53084.67 & --- & 53007.17 \\ \hline
        case2868rte & 0.01 & 1 & --- & 1 & --- & 0.14 & 21 & --- & 0.06 & 79908.26 & 79839.74 & --- & 79793.34 \\ \hline
		case6468rte & 0.01 & 5 & --- & 7 & --- & 0.33 & 21 & --- & 0.22 & 87097.02 & 87002.17 & --- & 86813.43 \\ \hline
        case6470rte & 0.01 & 1 & --- & 6 & --- & 0.17 & 23 & --- & 0.12 & 98503.85 & 98447.24 & --- & 98333.56 \\ \hline
        case6495rte & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  \\ \hline
        case6515rte & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  \\ \hline            
		\hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% pegase %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        case89pegase & 0.1 & 1 & --- & 21 & 0.00 & 0.00 & 21 & 0.00 & 0.00 & 5819.81 & 5819.81 & 5819.81 & 5819.67 \\
		\hline
        case1354pegase & 0.01 & 1 & --- & 1 & --- & 0.16 & 17 & --- & 0.08 & 74180.09 & 74121.53 & --- & 74062.53\\
		\hline
		case2869pegase & 0.01 & 1 & --- & 1 & 0.14 & 0.15 & 20 & 0.05 & 0.06 & 134187.63 & 134064.70 & 133999.84 & 133988.85 \\
		\hline
        case9241pegase & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
		\hline
        case13659pegase & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
		\hline
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% rte %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 		case1888rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case1951rte & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
%         case2848rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case2868rte & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- \\
% 		\hline
%         case6468rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case6470rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & --- \\
% 		\hline
%         case6495rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
% 		\hline
%         case6515rte & --- & --- & --- & --- & --- & --- & --- & ---& --- & --- & --- & ---  \\
%         \hline
%         \hline
	\end{tabular}
	\label{tab:SOCP_tb_1}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t] 
\scriptsize
	\centering
	\caption{SOCP results summary for NESTA test cases.}
	\begin{tabular}{ |c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Test Case} & \multicolumn{13}{c|}{SOCP}\\
		\cline{2-14}
 		& $\mu$ & $\alpha$ & t(s) & $k_{f}$ & \%GFB & \%GFS & $k_{p}$ & \%GPB & \%GPS & $c_{f}$ & $c_{p}$ & $c_{g}$ & $lb$\\
		\hline
		\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nesta %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 156.43 & 156.43 & 156.43 & 156.43 \\ \hline
        nesta\_case5\_pjm & 0.0001 & 1 & --- & 1 & 1.24 & 6.39 & 35 & 0.01 & 5.23 & 17771.60 & 17553.10 & 17551.89 & 16635.78 \\ \hline
        nesta\_case6\_c & 0.1 & 1 & --- & 1 & 3.25 & 3.25 & 3 & 0.17 & 0.17 & 23.99 & 23.25 & 23.21 & 23.21 \\ \hline
        nesta\_case9\_wscc & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 5296.69 & 5296.69 & 5296.69 & 5296.69 \\ \hline
        nesta\_case14\_ieee & 0.1 & 1 & --- & 1 & 0.11 & 0.11 & 5 & 0.00 & 0.00 & 244.31 & 244.05 & 244.05 & 244.05 \\ \hline
        nesta\_case24\_ieee\_rts & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 63352.23 & 63352.23 & 63352.20 & 63352.20 \\ \hline
        nesta\_case29\_edin & 0.1 & 1 & --- & 1 & 0.12 & 0.12 & 4 & 0.00 & 0.00 & 29929.97 & 29895.92 & 29895.49 & 29895.49 \\ \hline
        nesta\_case30\_as & 0.1 & 1 & --- & 1 & 0.39 & 0.39 & 3 & 0.00 & 0.00 & 806.30 & 803.14 & 803.13 & 803.13 \\ \hline
        nesta\_case30\_fsr & 0.1 & 1 & --- & 1 & 0.08 & 0.08 & 3 & 0.00 & 0.00 & 576.24 & 575.77 & 575.77 & 575.77 \\ \hline
        nesta\_case30\_ieee & 0.1 & 1 & --- & 1 & 0.27 & 0.27 & 3 & 0.00 & 0.00 & 205.53 & 204.97 & 204.97 & 204.97 \\ \hline
        nesta\_case39\_epri & 0.01 & 1 & --- & 2 & 0.00 & 0.02 & 2 & 0.00 & 0.02 & 96505.76 & 96505.76 & 96505.52 & 96491.10 \\ \hline
        nesta\_case57\_ieee & 0.1 & 1 & --- & 1 & 0.10 & 0.10 & 3 & 0.00 & 0.00 & 1144.41 & 1143.29 & 1143.27 & 1143.27 \\ \hline
        nesta\_case73\_ieee\_rts & 0.1 & 1 & --- & 1 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 189764.20 & 189764.20 & 189764.08 & 189764.08 \\ \hline
        nesta\_case89\_pegase & 0.1 & 1 & --- & 46 & 0.00 & 0.00 & 46 & 0.00 & 0.00 & 5819.81 & 5819.81 & 5819.81 & 5819.67 \\ \hline
        nesta\_case118\_ieee & 0.1 & 1 & --- & 1 & 2.34 & 2.40 & 8 & 0.00 & 0.07 & 3807.56 & 3718.74 & 3718.64 & 3716.25 \\ \hline
        \textcolor{orange}{nesta\_case162\_ieee\_dtc}& 0.01 & 5 & --- & 10 & 1.45 & 2.51 & 50 & 0.89 & 1.96 & 4292.47 & 4268.28 & 4230.23 & 4184.71 \\ \hline
        nesta\_case189\_edin& --- & --- & --- & ---  & ---  & --- & ---  & ---  & ---  & --- & ---  & ---  & ---  \\ \hline
        \textcolor{orange}{nesta\_case300\_ieee}& 0.01 & 1 & --- & 1 & 3.91 & 3.98 & 50 & 0.02 & 0.09 & 17578.10 & 16893.91 & 16891.28 & 16878.14 \\ \hline
		\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nesta_api %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs\_\_api & 0.01 & 1 & --- & 1 & -0.08 & 0.00 & 1 & -0.08 & 0.00 & 766.67 & 766.67 & 767.27 & 766.67 \\ \hline
        nesta\_case5\_pjm\_\_api & 0.1 & 5 & --- & 1 & -0.05 & 0.03 & 2 & -0.07 & 0.00 & 2997.11 & 2996.32 & 2998.54 & 2996.32 \\ \hline
        nesta\_case6\_c\_\_api & 0.1 & 1 & --- & 2 & -0.07 & 0.00 & 2 & -0.07 & 0.00 & 813.87 & 813.87 & 814.40 & 813.87 \\ \hline
        nesta\_case9\_wscc\_\_api & 0.1 & 5 & --- & 1 & -0.06 & 0.00 & 1 & -0.06 & 0.00 & 656.23 & 656.23 & 656.60 & 656.23 \\ \hline
        nesta\_case14\_ieee\_\_api & 0.1 & 5 & --- & 3 & -0.10 & 0.04 & 5 & -0.13 & 0.00 & 325.25 & 325.13 & 325.56 & 325.13 \\ \hline
        nesta\_case24\_ieee\_rts\_\_api & 0.01 & 5 & --- & 13 & 0.14 & 1.52 & 17 & 0.10 & 1.47 & 6430.53 & 6427.64 & 6421.37 & 6333.07 \\ \hline
        \textcolor{yellow}{nesta\_case29\_edin\_\_api} & 0.01 & 1 & --- & 1 & -0.08 & 0.08 & 3 & -0.16 & 0.01 & 295538.73 & 295318.14 & 295782.68 & 295291.22 \\ \hline
        nesta\_case30\_as\_\_api & 0.01 & 1 & --- & 2 & 0.61 & 0.80 & 6 & -0.18 & 0.00 & 574.65 & 570.09 & 571.13 & 570.08 \\ \hline
        nesta\_case30\_fsr\_\_api & 0.001 & 5 & --- & 1 & 4.18 & 15.56 & 38 & -1.46 & 10.59 & 388.36 & 366.79 & 372.14 & 327.95 \\ \hline
        nesta\_case30\_ieee\_\_api & 0.1 & 5 & --- & 5 & -0.13 & 0.00 & 5 & -0.13 & 0.00 & 414.99 & 414.99 & 415.53 & 414.99 \\ \hline
        nesta\_case39\_epri\_\_api & 0.1 & 1 & --- & 3 & -0.08 & 0.00 & 3 & -0.08 & 0.00 & 7460.37 & 7460.37 & 7466.25 & 7460.37 \\ \hline
        nesta\_case57\_ieee\_\_api & 0.1 & 1 & --- & 2 & 0.01 & 0.09 & 3 & 0.00 & 0.08 & 1430.76 & 1430.67 & 1430.65 & 1429.51 \\ \hline
        \textcolor{orange}{nesta\_case73\_ieee\_rts\_\_api}& 0.001 & 5 & --- & 3 & 2.11 & 6.92 & 50 & -0.04 & 4.87 & 20558.29 & 20115.87 & 20123.98 & 19135.79  \\ \hline
        nesta\_case89\_pegase\_\_api& --- & --- & --- & ---  & ---  & --- & ---  & ---  & ---  & --- & ---  & ---  & ---  \\ \hline
        nesta\_case162\_ieee\_dtc\_\_api & 0.001 & 1 & --- & 8 & 0.17 & 1.09 & 31 & -0.05 & 0.87 & 6122.12 & 6108.61 & 6111.68 & 6055.28 \\ \hline
        \textcolor{orange}{nesta\_case300\_ieee\_\_api}& 0.01 & 1 & --- & 1 & -8.45 & 5.77 & 50 & -15.02 & 0.06 & 21083.92 & 19879.19 & 22866.01 & 19866.78 \\ \hline
        \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nesta_sad %%%%%%%%%%%%%%%%%%%%%%%%%%
        nesta\_case4\_gs\_\_sad & 0.01 & 1 & --- & 1 & -2.59 & 0.05 & 1 & -2.59 & 0.05 & 315.84 & 315.84 & 324.02 & 315.69 \\ \hline
         \textcolor{yellow}{nesta\_case5\_pjm\_\_api} & 0.1 & 5 & --- & 1 & -0.05 & 0.03 & 2 & -0.07 & 0.00 & 2997.11 & 2996.32 & 2998.54 & 2996.32 \\ \hline
        nesta\_case6\_c\_\_sad & 0.1 & 1 & --- & 1 & 0.08 & 0.29 & 5 & -0.21 & 0.00 & 24.45 & 24.38 & 24.43 & 24.38 \\ \hline
        nesta\_case6\_ww\_\_sad & 0.1 & 5 & --- & 1 & -0.10 & 0.00 & 1 & -0.10 & 0.00 & 3146.27 & 3146.27 & 3149.51 & 3146.27 \\ \hline
        nesta\_case9\_wscc\_\_sad & 0.01 & 5 & --- & 1 & -1.11 & 0.01 & 2 & -1.12 & 0.00 & 5528.77 & 5528.26 & 5590.09 & 5528.26 \\ \hline
        nesta\_case14\_ieee\_\_sad & 0.1 & 1 & --- & 1 & 0.07 & 0.11 & 5 & -0.04 & 0.00 & 244.31 & 244.05 & 244.15 & 244.05 \\ \hline
        nesta\_case24\_ieee\_rts\_\_sad & 0.001 & 5 & --- & 1 & -3.55 & 4.51 & 2 & -3.72 & 4.36 & 77068.94 & 76943.63 & 79804.96 & 73591.73 \\ \hline
        nesta\_case29\_edin\_\_sad & 0.001 & 5 & --- & 6 & -13.34 & 20.74 & 26 & -13.70 & 20.48 & 41407.72 & 41276.51 & 46933.26 & 32821.76 \\ \hline
        nesta\_case30\_as\_\_sad & 0.01 & 1 & --- & 1 & -0.18 & 1.91 & 3 & -1.89 & 0.24 & 912.78 & 897.50 & 914.44 & 895.34 \\ \hline
        nesta\_case30\_fsr\_\_sad & 0.1 & 1 & --- & 1 & -0.14 & 0.04 & 2 & -0.16 & 0.02 & 576.90 & 576.79 & 577.73 & 576.68 \\ \hline
        nesta\_case30\_ieee\_\_sad & 0.1 & 1 & --- & 1 & 0.20 & 0.27 & 3 & -0.07 & 0.00 & 205.53 & 204.97 & 205.11 & 204.97 \\ \hline
        nesta\_case39\_epri\_\_sad & 0.01 & 1 & --- & 1 & -0.49 & 0.06 & 2 & -0.49 & 0.05 & 96749.21 & 96745.01 & 97219.04 & 96692.45 \\ \hline
        nesta\_case57\_ieee\_\_sad & 0.1 & 1 & --- & 1 & 0.05 & 0.10 & 3 & -0.05 & 0.00 & 1144.41 & 1143.29 & 1143.88 & 1143.27 \\ \hline
        nesta\_case73\_ieee\_rts\_\_sad & 0.001 & 5 & --- & 1 & -3.27 & 2.77 & 3 & -3.29 & 2.75 & 227797.80 & 227754.75 & 235241.70 & 221480.59 \\ \hline
		nesta\_case89\_pegase\_\_sad & 0.001 & 1 & --- & 1 & -0.00 & 0.12 & 1 & -0.00 & 0.12 & 5826.88 & 5826.88 & 5827.01 & 5819.67 \\ \hline
        nesta\_case118\_ieee\_\_sad & 0.1 & 5 & --- & 3 & -5.01 & 3.73 & 15 & -5.29 & 3.48 & 4117.93 & 4107.05 & 4324.17 & 3964.14 \\ \hline
        \textcolor{orange}{nesta\_case162\_ieee\_dtc\_\_sad}& 0.001 & 1 & --- & 3 & -0.29 & 3.58 & 50 & -1.77 & 2.15 & 4356.62 & 4293.00 & 4369.19 & 4200.52   \\ \hline
        \textcolor{orange}{nesta\_case189\_edin\_\_sad} & 0.001 & 1 & --- & 49 & 6.31 & 12.11 & 50 & 4.01 & 9.95 & 976.23 & 952.82 & 914.61 & 858.01  \\ \hline
        nesta\_case300\_ieee\_\_sad & 0.01 & 1 & --- & 1 & 3.76 & 3.93 & 49 & -0.08 & 0.09 & 17570.81 & 16896.67 & 16910.23 & 16880.74 \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\end{tabular}
	\label{tab:SOCP_tb_2}
\end{table*}
